The ELAPS Framework: Experimental Linear Algebra Performance Studies

Optimal use of computing resources requires extensive coding, tuning and benchmarking. To boost developer productivity in these time consuming tasks, we introduce the Experimental Linear Algebra Performance Studies framework (ELAPS), a multi-platform open source environment for fast yet powerful performance experimentation with dense linear algebra kernels, algorithms, and libraries. ELAPS allows users to construct experiments to investigate how performance and efficiency vary depending on factors such as caching, algorithmic parameters, problem size, and parallelism. Experiments are designed either through Python scripts or a specialized GUI, and run on the whole spectrum of architectures, ranging from laptops to clusters, accelerators, and supercomputers. The resulting experiment reports provide various metrics and statistics that can be analyzed both numerically and visually. We demonstrate the use of ELAPS in four concrete application scenarios and in as many computing environments, illustrating its practical value in supporting critical performance decisions.

==> Makefile <==
PDFLATEX = pdflatex -shell-escape -recorder

TARGET = main.pdf

TEXFILES = *.tex figures/*.tex

default: once

# internals below

TARGETSTEM = $(TARGET:.pdf=)

once: 
	$(PDFLATEX) $(TARGETSTEM)

twice:
	make once
	make once

figs:
	time make -j 4 -f $(TARGETSTEM).makefile

ffigs:
	time make -j 4 -f $(TARGETSTEM).makefile -B

bib:
	bibtex $(TARGETSTEM)

all:
	make once
	make figs
	make bib
	make once
	make ffigs
	make twice

bg:
	make once < /dev/null 2>&1 1> /dev/null &

check: $(TEXFILES)
	for file in $(TEXFILES); \
	do \
		aspell --lang=EN --mode=tex check $$file; \
	done

open:
	open $(TARGET)

clean:
	rm -rf $(TARGETSTEM).{blg,fls,aux,log,toc,pdf,lof,out,figlist,makefile,pyg} figures/externalized/*

